Reformulating van Rijsbergen's $F_{\beta}$ metric for weighted binary cross-entropy

The separation of performance metrics from gradient based loss functions may not always give optimal results and may miss vital aggregate information. This paper investigates incorporating a performance metric alongside differentiable loss functions to inform training outcomes. The goal is to guide model performance and interpretation by assuming statistical distributions on this performance metric for dynamic weighting. The focus is on van Rijsbergens $F_{\beta}$ metric -- a popular choice for gauging classification performance. Through distributional assumptions on the $F_{\beta}$, an intermediary link can be established to the standard binary cross-entropy via dynamic penalty weights. First, the $F_{\beta}$ metric is reformulated to facilitate assuming statistical distributions with accompanying proofs for the cumulative density function. These probabilities are used within a knee curve algorithm to find an optimal $\beta$ or $\beta_{opt}$. This $\beta_{opt}$ is used as a weight or penalty in the proposed weighted binary cross-entropy. Experimentation on publicly available data along with benchmark analysis mostly yields better and interpretable results as compared to the baseline for both imbalanced and balanced classes. For example, for the IMDB text data with known labeling errors, a 14% boost in $F_1$ score is shown. The results also reveal commonalities between the penalty model families derived in this paper and the suitability of recall-centric or precision-centric parameters used in the optimization. The flexibility of this methodology can enhance interpretation.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

%\bibitem{smoothF1} Bénédict, G., Koops, V., Odijk, D., and de Rijke, M. (2021). sigmoidF1: A Smooth F1 Score Surrogate Loss for Multilabel Classification. \textit{arXiv preprint arXiv:2108.10566.}

%\bibitem{bib20} Borisov, V., Leemann, T., Seßler, K., Haug, J., Pawelczyk, M., and Kasneci, G. (2021). Deep neural networks and tabular data: A survey. \textit{arXiv preprint arXiv:2110.01889.}

%\bibitem{smote} Chawla, N. V., Bowyer, K. W., Hall, L. O., and Kegelmeyer, W. P. (2002). SMOTE: synthetic minority over-sampling technique. \textit{Journal of artificial intelligence research, 16, 321-357.}

%\bibitem{bib6} Dua, D. and Graff, C. (2019). UCI Machine Learning Repository [http://archive.ics.uci.edu/ml]. Irvine, CA: University of California, School of Information and Computer Science.

%\bibitem{dud} Dudewicz, E. J., and Mishra, S. (1988). Modern mathematical statistics. John Wiley \& Sons, Inc.

%\bibitem{f1_3} Fujino, A., Isozaki, H., and Suzuki, J. (2008). Multi-label text categorization with model combination based on f1-score maximization. \textit{In Proceedings of the Third International Joint Conference on Natural Language Processing: Volume-II.}

%\bibitem{bib13} Grush, L. (2015). Google engineer apologizes after Photos app tags two black people as gorillas. \textit{The Verge, 1.}

%\bibitem{overundersample} Hasanin, T., Khoshgoftaar, T. M., Leevy, J. L., and Seliya, N. (2019). Examining characteristics of predictive models with imbalanced big data. \textit{Journal of Big Data, 6(1), 1-21.}

%\bibitem{bib7} He, K., Zhang, X., Ren, S., and Sun, J. (2016). Deep residual learning for image recognition. \textit{In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 770-778).}

%\bibitem{hogg} Hogg, R. V., and Craig, A. T. (1995). Introduction to mathematical statistics.(5"" edition). Englewood Hills, New Jersey.

%\bibitem{f1_2} Jansche, M. (2005, October). Maximum expected F-measure training of logistic regression models. \textit{In Proceedings of Human Language Technology Conference and Conference on Empirical Methods in Natural Language Processing (pp. 692-699).}

%\bibitem{bib17} Klie, J. C., Webber, B., and Gurevych, I. (2022). Annotation Error Detection: Analyzing the Past and Present for a More Coherent Future. \textit{arXiv preprint arXiv:2206.02280.}

%\bibitem{bib3} Lee, N., Yang, H., and Yoo, H., A surrogate loss function for optimization of $F_\beta $ score in binary classification with imbalanced data, \textit{arXiv preprint arXiv:2104.01459, 2021}.

%\bibitem{focal} Lin, T. Y., Goyal, P., Girshick, R., He, K., and Dollár, P. (2017). Focal loss for dense object detection. \textit{In Proceedings of the IEEE international conference on computer vision (pp. 2980-2988).}

%\bibitem{threshold} Lipton, Z. C., Elkan, C., and Narayanaswamy, B. (2014). Thresholding classifiers to maximize F1 score. \textit{arXiv preprint arXiv:1402.1892.}

%\bibitem{bib5} Maas, A., Daly, R. E., Pham, P. T., Huang, D., Ng, A. Y., and Potts, C., (June 2011) Learning word vectors for sentiment analysis. \textit{In Proceedings of the 49th annual meeting of the association for computational linguistics: Human language technologies (pp. 142-150).}

%\bibitem{recall2} Mohit, B., Schneider, N., Bhowmick, R., Oflazer, K., and Smith, N. A. (2012, April). Recall-oriented learning of named entities in Arabic Wikipedia. \textit{In Proceedings of the 13th Conference of the European Chapter of the Association for Computational Linguistics (pp. 162-173).}

%\bibitem{bib16} Northcutt, C. G., Athalye, A., and Mueller, J. (2021). Pervasive label errors in test sets destabilize machine learning benchmarks. \textit{arXiv preprint arXiv:2103.14749.}

%\bibitem{lrp} Oksuz, K., Cam, B. C., Akbas, E., and Kalkan, S. (2018). Localization recall precision (LRP): A new performance metric for object detection. \textit{In Proceedings of the European Conference on Computer Vision (ECCV) (pp. 504-519).}

%\bibitem{dice} Li, X., Sun, X., Meng, Y., Liang, J., Wu, F., and Li, J. (2019). Dice loss for data-imbalanced NLP tasks. \textit{arXiv preprint arXiv:1911.02855.}

%\bibitem{metriclikelrp} Ho, Y., and Wookey, S. (2019). The real-world-weight cross-entropy loss function: Modeling the costs of mislabeling. \textit{IEEE Access, 8, 4806-4813.}
%
%\bibitem{rankandlrp} Oksuz, K., Cam, B. C., Akbas, E., and Kalkan, S. (2020). A ranking-based, balanced loss function unifying classification and localisation in object detection. \textit{Advances in Neural Information Processing Systems, 33, 15534-15545.}
%
%\bibitem{bib12} Qian, S., Pham, V. H., Lutellier, T., Hu, Z., Kim, J., Tan, L., ... and Shah, S. (2021). Are my deep learning systems fair? An empirical study of fixed-seed training. \textit{Advances in Neural Information Processing Systems, 34, 30211-30227.}
%
%\bibitem{bib8} Sandler, M., Howard, A., Zhu, M., Zhmoginov, A., and Chen, L. C. (2018). Mobilenetv2: Inverted residuals and linear bottlenecks. \textit{In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 4510-4520).}
%
%\bibitem{bib2} Sasaki, Y., The Truth of the F-Measure, \textit{University of Manchester Technical Report, 2007.}
%
%\bibitem{bib4} Satopaa, V., Albrecht, J., Irwin, D., and Raghavan, B., Finding a \textit{kneedle} in a haystack: Detecting knee points in system behavior, \textit{In 2011 31st international conference on distributed computing systems workshops (pp. 166-171). IEEE}
%
%\bibitem{bib10} Schmidhuber, J. (2015). Deep learning in neural networks: An overview. \textit{Neural networks, 61, 85-117.}
%
%\bibitem{bib18} Song, H., Kim, M., Park, D., Shin, Y., and Lee, J. G. (2022). Learning from noisy labels with deep neural networks: A survey. \textit{IEEE Transactions on Neural Networks and Learning Systems.}
%
%\bibitem{bib19} Sun, B., Yang, L., Zhang, W., Lin, M., Dong, P., Young, C., and Dong, J. (2019). Supertml: Two-dimensional word embedding for the precognition on structured tabular data. \textit{In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (pp. 0-0).}
%
%\bibitem{recall} Tian, J., Mithun, N. C., Seymour, Z., Chiu, H. P., and Kira, Z. (2022, May). Striking the Right Balance: Recall Loss for Semantic Segmentation. \textit{In 2022 International Conference on Robotics and Automation (ICRA) (pp. 5063-5069). IEEE.}
%
%\bibitem{bib11} Tian, Y., Zhong, Z., Ordonez, V., Kaiser, G., and Ray, B. (2020, June). Testing dnn image classifiers for confusion \& bias errors. \textit{In Proceedings of the ACM/IEEE 42nd International Conference on Software Engineering (pp. 1122-1134).}
%
%\bibitem{bib15} Tian, Y. (2020, November). Repairing confusion and bias errors for DNN-based image classifiers. \textit{In Proceedings of the 28th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering (pp. 1699-1700).}
%
%\bibitem{bib1} Van Rijsbergen, C. J., Information retrieval 2nd, Newton MA, 1979.
%
%\bibitem{bib9} Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A. N., ... and Polosukhin, I. (2017). Attention is all you need. \textit{Advances in neural information processing systems, 30.}
%
%\bibitem{f1_1} Yan, B. C., Wang, H. W., Jiang, S. W. F., Chao, F. A., and Chen, B. (2022, July). Maximum f1-score training for end-to-end mispronunciation detection and diagnosis of L2 English speech. \textit{In 2022 IEEE International Conference on Multimedia and Expo (ICME) (pp. 1-5). IEEE.}
%
%\bibitem{bib14} Zhang, X., Zhai, J., Ma, S., and Shen, C. (2021, May). AUTOTRAINER: An Automatic DNN Training Problem Detection and Repair System. \textit{In 2021 IEEE/ACM 43rd International Conference on Software Engineering (ICSE) (pp. 359-371). IEEE.}
%
%\bibitem{bib21} Wen, B., Cao, Y., Yang, F., Subbalakshmi, K., and Chandramouli, R. (2022, March). Causal-TGAN: Modeling Tabular Data Using Causally-Aware GAN. \textit{In ICLR Workshop on Deep Generative Models for Highly Structured Data.}

\end{thebibliography}


